Testing the Physical Parameter Constraining Power of HCN and HNC with Neural Networks

We quantify the utility of HCN and HNC to characterize gas conditions in the nearby starburst galaxy NGC 253. We use measurements from the Atacama Large Millimeter/Submillimeter Array (ALMA) Large Program ALCHEMI: the ALMA Comprehensive High-resolution Molecular Inventory. Using different subsets of the eight total HCN and HNC transitions measured by ALCHEMI, we test the number and combinations of transitions necessary for constraining the temperature, H$_2$ volume and column densities, cosmic-ray ionization rate, and beam-filling factor in three representative regions within NGC 253. We use these combinations of HCN and HNC transitions to constrain chemical and radiative transfer models and infer the gas conditions using a Bayesian nested sampling algorithm combined with neural network models for increased efficiency. By comparing the shapes of the resulting posterior distributions, as well as the medians and uncertainties for each gas parameter, from each test case to what we obtain with the full set of eight transitions (the control), we quantify how well each test reproduces the control. We find that multiple transitions each of both molecules are required to obtain a median parameter value within a factor of 2 of the control with an uncertainty less than 2-3 times that of the control. We also find that transition combinations that feature a range of upper-state energies are most effective. We show that single transitions, such as HCN J = 1-0 or 3-2, are among the worst-performing combinations and result in parameter values up to an order of magnitude different than the control.

==> Notes.tex <==
% \begin{deluxetable*}{>{\scriptsize}c|>{\scriptsize}c|>{\scriptsize}l>{\scriptsize}l>{\scriptsize}l>{\scriptsize}l>{\scriptsize}l} 
% \tablecaption{Transition combination rankings with average percent difference between control and test medians, \%Diff$_\text{med}$, and ratio of test to control uncertainties, $\sigma_{\text{test}}/\sigma_\text{ctrl}$.\label{tab:mks}}
%     \tablehead{ \multicolumn{1}{c|}{\%Diff$_{\text{med}}$,} & \multicolumn{1}{c|}{Rank} & \multicolumn{1}{c}{$T_{\text{K}}$} & \multicolumn{1}{c}{$n_{\text{H}_{2}}$} & \multicolumn{1}{c}{$\zeta$} & \multicolumn{1}{c}{$N_{\text{H}_{2}}$} & \multicolumn{1}{c}{$\eta_{\text{ff}}$} \\
%     {\small $\sigma_{\text{test}}/\sigma_{\text{ctrl}}$}  & & & & & & }
%     \startdata
%     & 1 & \color{Purple4}\CIRCLE \space HCN $4-3$ + HNC & \color{VioletRed1}$\blacktriangle$ no HCN $1-0$ & \color{VioletRed1}$\blacktriangle$ no HCN $2-1$& \color{VioletRed1}$\blacktriangle$ no HCN $3-2$ & \color{VioletRed1}$\blacktriangle$ no HNC $2-1$\\
%     & 2 &  \color{VioletRed1}$\blacktriangle$ no HCN $2-1$ & \color{VioletRed1}$\blacktriangle$ no HCN $4-3$& \color{VioletRed1}$\blacktriangle$ no HCN $1-0$ & \color{VioletRed1}$\blacktriangle$ no HNC $4-3$ & \color{VioletRed1}$\blacktriangle$ no HCN $3-2$\\
%     & 3 &  \color{VioletRed1}$\blacktriangle$ no HNC $4-3$ & \color{VioletRed1}$\blacktriangle$ no HCN $2-1$ & \color{Purple4}\CIRCLE\space HCN $4-3$ + HNC & \color{VioletRed1}$\blacktriangle$ no HCN $1-0$ & \color{VioletRed1}$\blacktriangle$ no HCN $4-3$\\
%     & 4 &  \color{VioletRed1}$\blacktriangle$ no HNC $1-0$ & \color{SpringGreen4}{\ding{53}} $1-0$, $2-1$, $3-2$& \color{SpringGreen4}{\ding{53}} $1-0$, $2-1$, $3-2$& \color{SpringGreen4}{\ding{53}} $1-0$, $2-1$, $3-2$ & \color{VioletRed1}$\blacktriangle$ no HCN $2-1$\\
%     $<20$\%, & 5 &  \color{SpringGreen4}{\ding{53}} $1-0$, $2-1$, $4-3$ & \color{Purple4}\CIRCLE\space HCN $4-3$ + HNC & \color{VioletRed1}$\blacktriangle$ no HNC $2-1$ & \color{VioletRed1}$\blacktriangle$ no HCN $4-3$ & \color{SpringGreen4}{\ding{53}} $1-0$, $3-2$, $4-3$\\
%     $<$1.35& 6 &  \color{VioletRed1}$\blacktriangle$ no HCN $1-0$ &\color{VioletRed1}$\blacktriangle$ no HNC $2-1$ & \color{VioletRed1}$\blacktriangle$ no HNC $3-2$& \color{VioletRed1}$\blacktriangle$ no HNC $3-2$ & \color{SpringGreen4}{\ding{53}} $1-0$, $4-3$\\
%     & 7 &  \color{VioletRed1}$\blacktriangle$ no HCN $4-3$ & \color{Purple4}\CIRCLE\space HCN $1-0$ + HNC & \color{SpringGreen4}{\ding{53}} $1-0$, $4-3$& \color{Purple4}\CIRCLE\space HNC $1-0$ + HCN & \color{SpringGreen4}{\ding{53}} $1-0$, $2-1$, $3-2$\\
%     & 8 &  \color{SpringGreen4}{\ding{53}} $1-0$, $4-3$ & \color{SpringGreen4}{\ding{53}} $1-0$, $4-3$& \color{SpringGreen4}{\ding{53}} $1-0$, $3-2$, $4-3$ & \color{SpringGreen4}{\ding{53}} $1-0$, $3-2$, $4-3$ & \color{RoyalBlue3}$\blacksquare$ HNC only\\
%     & 9 &  \color{VioletRed1}$\blacktriangle$ no HNC $3-2$ &\color{Purple4}\CIRCLE\space HNC $1-0$ + HCN &\color{SpringGreen4}{\ding{53}} $1-0$, $3-2$ & \color{VioletRed1}$\blacktriangle$ no HNC $1-0$ & \color{VioletRed1}$\blacktriangle$ no HNC $3-2$\\
%     \hline
%     & 10 & \color{SpringGreen4}{\ding{53}} $1-0$, $3-2$, $4-3$ & \color{SpringGreen4}{\ding{53}} $1-0$, $3-2$, $4-3$ &\color{Purple4}\CIRCLE\space HNC $1-0$ + HCN & \color{Purple4}\CIRCLE\space HCN $4-3$ + HNC & \color{Purple4}\CIRCLE\space HCN $4-3$ + HNC\\
%      & 11 & \color{Purple4}\CIRCLE\space HNC $4-3$ + HCN & \color{VioletRed1}$\blacktriangle$ no HCN $3-2$&\color{VioletRed1}$\blacktriangle$ no HCN $3-2$ & \color{SpringGreen4}{\ding{53}} $1-0$, $2-1$, $4-3$ & \color{VioletRed1}$\blacktriangle$ no HNC $1-0$\\
%      & 12 & \color{VioletRed1}$\blacktriangle$ no HCN $3-2$ & \color{RoyalBlue3}$\blacksquare$ HNC only& \color{Purple4}\CIRCLE\space HCN $1-0$ + HNC& \color{RoyalBlue3}$\blacksquare$ HNC only  & \color{VioletRed1}$\blacktriangle$ no HCN $1-0$\\
%     $<60$\%,& 13 & \color{Sienna3}$\blacklozenge$ HCN $4-3$ & \color{SpringGreen4}{\ding{53}} $1-0$, $2-1$, $4-3$ & \color{VioletRed1}$\blacktriangle$ no HNC $1-0$ &  \color{SpringGreen4}{\ding{53}} $1-0$, $3-2$  & \color{Purple4}\CIRCLE\space HNC $4-3$ + HCN\\
%      $<2.1$ & 14 & \color{SpringGreen4}{\ding{53}} $1-0$, $2-1$, $3-2$ & \color{SpringGreen4}{\ding{53}} $1-0$, $3-2$ & \color{SpringGreen4}{\ding{53}} $1-0$, $2-1$, $4-3$& \color{SpringGreen4}{\ding{53}} $1-0$, $4-3$ & \color{SpringGreen4}{\ding{53}} $1-0$, $3-2$\\
%     & 15 & \color{SpringGreen4}{\ding{53}} $3-2$, $4-3$& \color{VioletRed1}$\blacktriangle$ no HNC $4-3$& \color{VioletRed1}$\blacktriangle$ no HNC $4-3$ & \color{Purple4}\CIRCLE\space HCN $1-0$ + HNC & \color{RoyalBlue3}$\blacksquare$ HCN only\\
%     & 16 & \color{Purple4}\CIRCLE\space HNC $1-0$ + HCN &\color{Sienna3}$\blacklozenge$ HNC $4-3$ &  \color{VioletRed1}$\blacktriangle$ no HCN $4-3$& \color{VioletRed1}$\blacktriangle$ no HNC $2-1$& \color{Purple4}\CIRCLE\space HNC $1-0$ + HCN\\
%      & 17 & \color{Sienna3}$\blacklozenge$ HCN $3-2$ & \color{Sienna3}$\blacklozenge$ HNC $3-2$ & \color{Purple4}\CIRCLE\space HNC $4-3$ + HCN & \color{SpringGreen4}{\ding{53}} $1-0$, $2-1$& \color{SpringGreen4}{\ding{53}} $2-1$, $3-2$, $4-3$\\
%     & 18 & \color{RoyalBlue3}$\blacksquare$ HNC only & \color{VioletRed1}$\blacktriangle$ no HNC $1-0$ & \color{SpringGreen4}{\ding{53}} $3-2$, $4-3$& \color{RoyalBlue3}$\blacksquare$ HCN only & \color{SpringGreen4}{\ding{53}} $2-1$, $4-3$\\
%     \hline
%     & 19 & \color{VioletRed1}$\blacktriangle$ no HNC $2-1$ & \color{SpringGreen4}{\ding{53}} $2-1$ & \color{SpringGreen4}{\ding{53}} $1-0$& \color{Sienna3}$\blacklozenge$ HNC $1-0$& \color{Purple4}\CIRCLE\space HCN $1-0$ + HNC\\
%     & 20 & \color{Sienna3}$\blacklozenge$ HCN $2-1$ & \color{SpringGreen4}{\ding{53}} $1-0$, $2-1$ & \color{SpringGreen4}{\ding{53}} $3-2$& \color{SpringGreen4}{\ding{53}} $1-0$ & \color{SpringGreen4}{\ding{53}} $3-2$, $4-3$\\
%     & 21 & \color{Sienna3}$\blacklozenge$ HNC $3-2$ & \color{RoyalBlue3}$\blacksquare$ HCN only & \color{SpringGreen4}{\ding{53}} $4-3$& \color{Sienna3}$\blacklozenge$ HCN $3-2$ & \color{SpringGreen4}{\ding{53}} $1-0$, $2-1$, $4-3$\\
%     $<250$\%, & 22 & \color{SpringGreen4}{\ding{53}} $4-3$ & \color{Sienna3}$\blacklozenge$ HNC $2-1$ &\color{SpringGreen4}{\ding{53}} $2-1$ & \color{Purple4}\CIRCLE\space HNC $4-3$ + HCN& \color{SpringGreen4}{\ding{53}} $2-1$, $3-2$\\
%     $<7.5$& 23 & \color{SpringGreen4}{\ding{53}} $2-1$ & \color{SpringGreen4}{\ding{53}} $3-2$, $4-3$ &\color{Sienna3}$\blacklozenge$ HNC $4-3$ & \color{Sienna3}$\blacklozenge$ HNC $3-2$& \color{SpringGreen4}{\ding{53}} $1-0$, $2-1$\\
%     & 24 & \color{SpringGreen4}{\ding{53}} $2-1$, $4-3$ & \color{Purple4}\CIRCLE\space HNC $4-3$ + HCN & \color{Sienna3}$\blacklozenge$ HNC $3-2$& \color{SpringGreen4}{\ding{53}} $3-2$, $4-3$& \color{Sienna3}$\blacklozenge$ HNC $4-3$\\
%     & 25 & \color{SpringGreen4}{\ding{53}} $1-0$, $3-2$ & \color{Sienna3}$\blacklozenge$ HCN $2-1$ & \color{SpringGreen4}{\ding{53}} $1-0$, $2-1$& \color{SpringGreen4}{\ding{53}} $2-1$, $3-2$& \color{Sienna3}$\blacklozenge$ HNC $2-1$\\
%     & 26 & \color{RoyalBlue3}$\blacksquare$ HCN only & \color{Sienna3}$\blacklozenge$ HCN $4-3$ &\color{SpringGreen4}{\ding{53}} $2-1$, $3-2$, $4-3$ & \color{Sienna3}$\blacklozenge$ HCN $2-1$& \color{Sienna3}$\blacklozenge$ HNC $1-0$\\
%     & 27 & \color{Sienna3}$\blacklozenge$ HCN $1-0$ & \color{VioletRed1}$\blacktriangle$ no HNC $3-2$ &\color{Sienna3}$\blacklozenge$ HNC $1-0$ &\color{Sienna3}$\blacklozenge$ HCN $4-3$ & \color{VioletRed1}$\blacktriangle$ no HNC $4-3$\\
%     \hline
%     & 28 & \color{Sienna3}$\blacklozenge$ HNC $4-3$ & \color{SpringGreen4}{\ding{53}} $4-3$ & \color{Sienna3}$\blacklozenge$ HNC $2-1$ &\color{Sienna3}$\blacklozenge$ HCN $1-0$ &\color{Sienna3}$\blacklozenge$ HNC $3-2$ \\
%     & 29 & \color{Sienna3}$\blacklozenge$ HNC $1-0$ & \color{SpringGreen4}{\ding{53}} $1-0$ &\color{SpringGreen4}{\ding{53}} $2-1$, $3-2$& \color{SpringGreen4}{\ding{53}} $2-1$, $3-2$, $4-3$& \color{Sienna3}$\blacklozenge$ HCN $3-2$\\
%     & 30 & \color{Purple4}\CIRCLE\space HCN $1-0$ + HNC & \color{SpringGreen4}{\ding{53}} $3-2$ & \color{Sienna3}$\blacklozenge$ HCN $4-3$& \color{SpringGreen4}{\ding{53}} $3-2$& \color{Sienna3}$\blacklozenge$ HCN $2-1$\\
%     $250-500$\%, & 31 & \color{Sienna3}$\blacklozenge$ HNC $2-1$ & \color{Sienna3}$\blacklozenge$ HNC $1-0$ & \color{Sienna3}$\blacklozenge$ HCN $3-2$& \color{SpringGreen4}{\ding{53}} $2-1$, $4-3$& \color{Sienna3}$\blacklozenge$ HCN $1-0$\\
%     $7.5-16$& 32 & \color{SpringGreen4}{\ding{53}} $3-2$ & \color{SpringGreen4}{\ding{53}} $2-1$, $3-2$, $4-3$ &\color{Sienna3}$\blacklozenge$ HCN $1-0$ &\color{SpringGreen4}{\ding{53}} $2-1$ & \color{SpringGreen4}{\ding{53}} $2-1$ \\
%     & 33 & \color{SpringGreen4}{\ding{53}}   $2-1$, $3-2$, $4-3$ & \color{Sienna3}$\blacklozenge$ HCN $3-2$ & \color{RoyalBlue3}$\blacksquare$ HCN only & \color{SpringGreen4}{\ding{53}} $4-3$& \color{SpringGreen4}{\ding{53}} $4-3$\\
%     & 34 & \color{SpringGreen4}{\ding{53}}   $1-0$, $2-1$ & \color{Sienna3}$\blacklozenge$ HCN $1-0$& \color{Sienna3}$\blacklozenge$ HCN $2-1$& \color{Sienna3}$\blacklozenge$ HNC $2-1$& \color{Sienna3}$\blacklozenge$ HCN $4-3$\\
%     & 35 & \color{SpringGreen4}{\ding{53}}   $2-1$, $3-2$ & \color{SpringGreen4}{\ding{53}} $2-1$, $4-3$ & \color{SpringGreen4}{\ding{53}} $2-1$, $4-3$& \color{Sienna3}$\blacklozenge$ HNC $4-3$& \color{SpringGreen4}{\ding{53}} $1-0$\\
%     & 36 & \color{SpringGreen4}\ding53   $1-0$ & \color{SpringGreen4}{\ding{53}} $2-1$, $3-2$& \color{RoyalBlue3}$\blacksquare$ HNC only& \color{VioletRed1}$\blacktriangle$ no HCN $2-1$ & \color{SpringGreen4}{\ding{53}} $3-2$\\
%    \enddata
% \tablenotetext{\color{Sienna3}\blacklozenge}{ \color{Sienna3} Single HCN OR HNC transition (1 transition)}
% \tablenotetext{$\color{SpringGreen4}\ding{53}$}{ \color{SpringGreen4}Matched HCN and HNC transitions (2--6 transitions)}
% \tablenotetext{\color{RoyalBlue3}\blacksquare}{ \color{RoyalBlue3}All HCN OR all HNC transitions (4 transitions)}
% \tablenotetext{\color{Purple4}\CIRCLE}{ \color{Purple4}All HCN with one HNC transition OR all HNC with one HCN transition (5 transitions)}
% \tablenotetext{\color{VioletRed1}\blacktriangle}{ \color{VioletRed1}Single HCN or HNC transition removed (7 transitions)}
% \end{deluxetable*}



%\subsubsection{Test Combination Ranking} \label{sec:mks_ranking}

%To more easily compare the effectiveness of various combinations of HCN and HNC transitions in constraining gas physical parameters, we develop a comprehensive ranking system based on the posterior distribution residuals. In this system, each combination is assigned a score based on its placement in the ordered lists of residuals shown in Figures~\ref{fig:reg26_resids}, \ref{fig:reg53_resids}, and , \ref{fig:reg51_resids} for a certain gas parameter within a given region. Transition combinations with the lowest (best) residual values for a given gas parameter within a particular region are assigned a score of 1, and the combinations with the highest (worst) residuals out of the 36 combinations are given a score of 36. For each parameter, the transition combination scores from each of the three regions are summed, ultimately providing a list of scored transition combinations for each gas parameter, where a lower score corresponds to a better reproduction of the control distributions. The combination with the lowest overall score across all 3 regions for a given parameter is assigned a rank of 1, the second-scoring transition combination for that parameter is given a rank of 2, and so on.
%We thus use these total scores to rank the transition combinations from best to worst for each gas parameter, as seen in Table~\ref{tab:mks}. We have also added metrics in Table~\ref{tab:mks} to aid the reader in understanding how well combinations of various rankings perform in constraining the gas conditions. These metrics show what the percent difference is between the control and test medians (\%Diff$_{\text{med}}$), as well as the ratio of the test and control uncertainties, $\sigma_{\text{test}}/\sigma_{\text{ctrl}}$. Both of these metrics are averaged across all parameters and rankings within each subgroup shown.

% \begin{deluxetable*}{>{\scriptsize}c|>{\scriptsize}l|>{\scriptsize}l|>{\scriptsize}l} 
% \tablecaption{Transition Combinations that Meet Median and Uncertainty Criteria \label{tab:tList}}
%     \tablehead{ \multicolumn{1}{c|}{ } & \multicolumn{3}{c}{Region} \\
%     \cline{2-4}
%       & \multicolumn{1}{c|}{26} & \multicolumn{1}{c|}{51} & \multicolumn{1}{c}{53}
%      }
%     \startdata
%    $T_{\text{K}}$ & $\blacklozenge$: {\scriptsize HCN $4-3$\tablenotemark{*}} & $\blacklozenge$: None & \\
%                   & \ding{53}: $1-0$, $3-2$\tablenotemark{*} $\vert$  $1-0$, $4-3$\tablenotemark{*} $\vert$ $2-1$, $4-3$\tablenotemark{*}  & \ding{53}: $4-3$ $\vert$ $1-0$, $3-2$ $\vert$ $1-0$, $4-3$  & \\
%                   & $\space$ $\space$ $\space$ $\space$ $\space$ \scriptsize $1-0$, $2-1$, $4-3$ $\vert$ $1-0$, $3-2$, $4-3$\tablenotemark{*}  & $\space$ $\space$ $\space$ $\space$ $2-1$, $3-2$ $\vert$ $2-1$, $4-3$ $\vert$ $1-0$, $2-1$, $3-2$& \\
%                   & $\blacksquare$: all &  $\space$ $\space$ $\space$ $\space$ $1-0$, $2-1$, $4-3$ $\vert$ $1-0$, $3-2$, $4-3$& \\
%                   &  \CIRCLE: HCN $1-0$ + HNC\tablenotemark{*} $\vert$ HCN $4-3$ + HNC &  $\space$ $\space$ $\space$ $\space$ $2-1$, $3-2$, $4-3$ & \\
%                   & $$ $$ $$ $$ $$ $$HNC $1-0$ + HCN\tablenotemark{*} $\vert$ HNC $4-3$ + HCN\tablenotemark{*} &  $\blacksquare$: HCN only   &    \\ 
%                   &  $\blacktriangle$: all\tablenotemark{\scriptsize a} & \CIRCLE: HCN $4-3$ + HNC $\vert$ HNC $1-0$ + HCN & \\
%                   &  &  $\space$ $\space$ $\space$ $\space$ HNC $4-3$ + HCN & \\
%                   &  &  $\blacktriangle$: all & \\
%                   \hline
%    $n_{\text{H}_{2}}$ & $\blacklozenge$: {\scriptsize None} &  & \\ 
%                   & \ding{53}: {\scriptsize $1-0$, $2-1$\tablenotemark{*}} $\vert$ {\scriptsize $1-0$, $4-3$\tablenotemark{*}}& & \\
%                   & $$ $$ $$ $$ $$ $${\scriptsize $1-0$, $2-1$, $3-2$} $\vert$ {\scriptsize $1-0$, $2-1$, $4-3$\tablenotemark{*}} & & \\
%                   & $\blacksquare$: {\scriptsize HNC only\tablenotemark{*}} & & \\
%                   &  \CIRCLE: {\scriptsize HCN $1-0$ + HNC} $\vert$ {\scriptsize HCN $4-3$ + HNC} & & \\
%                   &  $\blacktriangle$: {\scriptsize no HCN $1-0$} $\vert$ {\scriptsize no HCN $2-1$} $\vert$
%                    {\scriptsize no HCN $3-2$}& & \\
%                    & $$ $$ $$ $$ $$$${\scriptsize no HCN $4-3$} $\vert$ {\scriptsize no HNC $3-2$\tablenotemark{*}} $\vert$ {\scriptsize no HNC $4-3$} & & \\
%                   \hline
%    $\zeta$        & $\blacklozenge$: {\scriptsize None}    & & \\ 
%                   & \ding{53}: {\scriptsize $1-0$, $3-2$\tablenotemark{*}} $\vert$ {\scriptsize $1-0$, $3-2$, $4-3$\tablenotemark{*}} & & \\
%                   & $\blacksquare$: {\scriptsize None} & & \\
%                   &  \CIRCLE: {\scriptsize None} & & \\
%                   & $\blacktriangle$: {\scriptsize no HCN $1-0$} $\vert$ {\scriptsize no HCN $2-1$} $\vert$ {\scriptsize no HCN $3-2$} & & \\
%                   & $$ $$ $$ $$ $$$${\scriptsize no HCN $4-3$} $\vert$ {\scriptsize no HNC $2-1$\tablenotemark{*}} $\vert$ {\scriptsize no HNC $3-2$\tablenotemark{*}} & & \\
%    \hline
%    $N_{\text{H}_{2}}$ & $\blacklozenge$: {\scriptsize None} & & \\
%                   & \ding{53}: {\scriptsize $1-0$, $2-1$, $3-2$} $\vert$ {\scriptsize $1-0$, $2-1$, $4-3$\tablenotemark{*}}& & \\
%                   & $\blacksquare$: {\scriptsize None} & & \\
%                   &  \CIRCLE: {\scriptsize HCN $1-0$ + HNC\tablenotemark{*}} $\vert$ {\scriptsize HCN $4-3$ + HNC} & & \\
%                   & $\blacktriangle$: {\scriptsize no HCN $1-0$} $\vert$ {\scriptsize no HCN $2-1$} $\vert$ {\scriptsize no HCN $3-2$} & & \\
%                   & $$ $$ $$ $$ $$$${\scriptsize no HCN $4-3$} $\vert$ {\scriptsize no HNC $3-2$\tablenotemark{*}} $\vert$ {\scriptsize no HNC $4-3$} & & \\
%    \hline
%    $\eta_{\text{ff}}$ & $\blacklozenge$: {\scriptsize None} & & \\
%                   & \ding{53}: {\scriptsize $1-0$, $3-2$} $\vert$ {\scriptsize $1-0$, $4-3$} $\vert$ 
%                   {\scriptsize $1-0$, $2-1$, $3-2$} & & \\
%                   & $$ $$ $$ $$ $$ $${\scriptsize $1-0$, $2-1$, $4-3$} $\vert$ {\scriptsize $1-0$, $3-2$, $4-3$} & & \\
%                   & $\blacksquare$: {\scriptsize HCN only} & & \\
%                   &  \CIRCLE: {\scriptsize HNC $1-0$ + HCN} $\vert$ {\scriptsize HNC $4-3$ + HCN} & & \\
%                   & $\blacktriangle$: {\scriptsize no HCN $2-1$} $\vert$ {\scriptsize no HCN $3-2$} $\vert$ {\scriptsize no HCN $4-3$} & & \\
%                   & $$ $$ $$ $$ $$$${\scriptsize no HNC $1-0$\tablenotemark{*}} $\vert$ {\scriptsize no HNC $2-1$} $\vert$ {\scriptsize no HNC $3-2$} & & \\
%                   & $$ $$ $$ $$ $$$${\scriptsize no HNC $4-3$} & & \\
%    \enddata
% \vspace{-2mm}
% \tablenotetext{\scriptstyle *}{\scriptsize $r>$ Q1}
% \vspace{-2mm}
% \tablenotetext{\scriptstyle a}{\scriptsize no HNC $2-1$ has $r>$ Q1}
% \vspace{-2mm}
% \tablenotetext{\scriptstyle \blacklozenge}{\scriptsize Single HCN OR HNC transition}
% \vspace{-2mm}
% \tablenotetext{\scriptstyle $\ding{53}$}{\scriptsize Matched HCN and HNC transitions}
% \vspace{-2mm}
% \tablenotetext{\scriptstyle \blacksquare}{\scriptsize All HCN OR all HNC transitions}
% \vspace{-2mm}
% \tablenotetext{\scriptstyle \CIRCLE}{\scriptsize All HCN with one HNC transition OR all HNC with one HCN transition}
% \vspace{-2mm}
% \tablenotetext{\scriptstyle \blacktriangle}{\scriptsize Single HCN or HNC transition removed}
% \end{deluxetable*}
